Geometric Path Enumeration for Equivalence Verification of Neural Networks

As neural networks (NNs) are increasingly introduced into safety-critical domains, there is a growing need to formally verify NNs before deployment. In this work we focus on the formal verification problem of NN equivalence which aims to prove that two NNs (e.g. an original and a compressed version) show equivalent behavior. Two approaches have been proposed for this problem: Mixed integer linear programming and interval propagation. While the first approach lacks scalability, the latter is only suitable for structurally similar NNs with small weight changes. The contribution of our paper has four parts. First, we show a theoretical result by proving that the epsilon-equivalence problem is coNP-complete. Secondly, we extend Tran et al.'s single NN geometric path enumeration algorithm to a setting with multiple NNs. In a third step, we implement the extended algorithm for equivalence verification and evaluate optimizations necessary for its practical use. Finally, we perform a comparative evaluation showing use-cases where our approach outperforms the previous state of the art, both, for equivalence verification as well as for counter-example finding.

==> abstract.tex <==
- Formal Verification of neural networks
    -> Equivalence verification
        -> Necessary for example for the compression of safety-critical neural networks

Currently: based on exact MILP encodings, which lack scalability, or interval propagation, which is impractical for structurally different or retrained networks.

Our work has the following parts:
    1. We show the coNP-completeness of the epsilon-equivalence problem for neural networks
    2. We extend Tran et al.'s geometric path enumeration to a setting with multiple neural networks
    3. We apply the extended algorithm to equivalence verification and evaluate optimizations necessary for practical usage
    4. Finally, evaluation ACAS Xu and modified MNIST benchmarks shows that NNEquiv can prove equivalence in cases where previous approaches like MilpEquiv and ReluDiff time out. +  Counterexamples
    
    
As neural networks (NNs) are increasingly introduced into safety-critical domains, there is a rising need to formally verify NNs before deployment.
In this work we focus on the verification problem of NN equivalence, which tries to prove that two networks (e.g. an original and a compressed version) show equivalent behavior.
For this problem there currently exist two approaches.
While Mixed Integer Linear Programming encodings of the problem lack scalability, interval propagation techniques \textbf{are only suitable for NNs with minor weight chances}.

The work in our paper has four parts.
First, we show a theoretical result by proving that the epsilon-equivalence problem is coNP-complete.
Secondly, we extend Tran et al.'s single NN geometric path enumeration algorithm to a setting with multiple NNs.
In a third step, we implement and apply the extended algorithm to equivalence verification and evaluate optimizations necessary for its practical use.
Finally, we perform a comparative evaluation showing use-cases where our implementation, NNEquiv, outperforms the previous State of the Art, both, in equivalence verification as well as in counter-example finding.

==========================================================

An increasing trend in applying neural networks to safety-critical domains necessitates their formal verification. One important property in this context is neural network equivalence, because networks are oftentimes compressed to fit computational and space restrictions of embedded systems. Existing techniques for the equivalence verification of neural networks are either based on exact MILP encodings, which lack scalability, or interval propagation, which is impractical for structurally different or retrained networks.

First, we provide a proof that the epsilon-equivalence problem for neural networks is coNP-complete, then we present NNEquiv - a novel technique to verify the equivalence of neural networks which extends Tran et al.'s geometric path enumeration approach. We optimize our method through over-approximations as well as branching and refinement heuristics. An evaluation on ACAS Xu and modified MNIST benchmarks shows that NNEquiv can prove equivalence in cases where previous approaches like MilpEquiv and ReluDiff time out.

==> old/sections/branch_tree_exploration.tex <==
\todo{Define exact Zonotope GPE before this chapter}
Given we introduced over-approximations over $\relu$ splits, it becomes necessary to define a strategy that decides which over-approximations are refined if it turns out that the property cannot be established with the current over-approximation.
The problem of refinement heuristics has been previously studied for single networks by \textcite{10.1007/978-3-030-76384-8_2} who showed that a classic refinement loop approach which over-approximates everything and step by step refines over-approximations starting at the beginning of the network performs poorer than exact analysis.
We were able to reproduce this behavior also for the case of equivalence verification with two networks.
The main reason for this behavior is the duplicate work that is necessary as the Zonotopes or Star Sets are propagated through the network multiple times with varying approximation depth.
Instead of always refining the first encountered $\relu$ node we also explored various other refinement heuristics which tried to decrease the necessary time by making a better decision about which node to split.
However, it turned out that all strategies suffered from at least one of the problems:
\begin{itemize}
    \item The computation of the decision is too costly and can thus not reduce solving times
    \item The decision procedure cannot distinguish between actual split neurons and ghost splits which are only a result of previous over-approximations.
\end{itemize}
It thus seemed the best idea to begin the computation with an exact strategy which splits on every encountered neuron, which, however, eventually transitions into over-approximation.
While this can, in principle, significantly reduce the necessary solving time it becomes necessary to find a suitable strategy which decides when to transition to over-approximation mode.
\textcite{10.1007/978-3-030-76384-8_2} previously evaluated a number of strategies for this problem, however, their results were fine-tuned for the ACAS Xu single network use case.
%While using an average might still be transferable to our use case, the fixed thresholds certainly do not generalize to other problem instances.
Generally speaking, the above described strategy problem can be described as a (partial) tree exploration problem.
\subsection{NEW}
For given networks $\mathcal{R},\mathcal{T}$ and an input space $I$ we define a tree $T$ consisting of all branches the exact Zonotope GPE algorithm explores for its equivalence verification.
We denote $T=\left(V,l,r\right)$ as the tree where $V$ corresponds to the inner nodes and leafs of the tree and $l,r:V\to V\cupplus\left\{\bot\right\}$ denote left and right successors of some node in $V$ such that the structure induced by $V,l$ and $r$ produces a binary tree with some root $S$.
Further, $V$ can be partitioned into $V=N\cupplus R \cupplus W$ where $N$ corresponds to the inner nodes with $\forall v \in N. l\left(v\right)\neq \bot \neq r\left(v\right) \land l\left(v\right)\neq r\left(v\right)$ and $R$ (resp. $W$) corresponds to the feasible (resp. infeasible) leafs $\forall v \in R \cupplus W. l\left(v\right) = r\left(v\right) = \bot$.
An exact execution of GPE implicitly produces a set of paths of the form $p \in N^*\times\left(R \cupplus W\right)$ that are explored sequentially.
This can be written as $P=\left\{p_1, \dotsi, p_{\left|R \cupplus W\right|}\right\}$.
Note that the number of paths produced is fixed to the number of feasible or infeasible leafs.
Additionally it is worth noting that every leaf can be mapped to a subset of the input space which is being verified on this leaf, i.e. we can define a function $A: R \cupplus W \to 2^I$ which maps a leaf to a subset of $I$ (in particular $\forall w \in W. A\left(w\right)=\emptyset$).
We can then lift this function to all nodes in $V$ by defining $A$ for all nodes in $N$ through $A\left(v\right) = A\left(l\left(v\right)\right) \cup A\left(r\left(v\right)\right)$.
In this case the root node of the tree $S \in N$ must fulfill $I \subseteq A\left(S\right)$.

The time taken to verify using exact Zonotope GPE is bounded through:
\[
\mathcal{O}\left( \left|P\right|*t_{\text{check}} + \sum_{p \in P} \left|p\right|*t_{\text{descend}} \right)
\]
Essentially, there is only one way in which we can speed up computation time for GPE:
By finding a tree $T'$ which has a smaller number of leafs $\left|R'\cupplus W'\right|$ or less deep paths $\left|p\right|$, but is also equivalent to $T$ in the sense that the root node $S'$ of $T'$ also has the property $I \subseteq A\left(S\right)$.
However, the problem is further complicated by the property which we want to prove.
Otherwise, we could otherwise simply choose a one leaf tree which covers all of $I$.
For a given equivalence property $\mathcal{E}$ we can thus define a function $\min_{\mathcal{E}}:N^*\times\left(R \cupplus W\right) \to \mathbb{N}$ which returns the number of necessary steps in the given path $p$ for the property $\mathcal{E}$ to be verifiable on $A\left(p_{\min_{\mathcal{E}}\left(p\right)}\right)$.
The exploration of the tree induced by the set of paths
\[
P^*=\left\{ p' \in N^*\times\left(R \cupplus W\right) | \exists p \in P: p'=p_{0 : \min_{\mathcal{E}}\left(p\right)}\right\}
\]
would then be sufficient to prove equivalence ($p_{0:\min_{\mathcal{E}}\left(p\right)}$ denotes the prefix path of $p$ from step $0$ to step $\min_{\mathcal{E}}\left(p\right)$).
While $\left|P\right|$ is the upper bound for the number of paths we have to consider, $\left|P^*\right|$ is the lower bound (in this work we omit the option of reordering the inner nodes of the tree which could, potentially further compress the tree).
Since GPE still needs to process the nodes on which no split is performed (i.e. it needs to compute the overapproximation), we denote the cost of this processing as $t_{\text{overapprox}}$ which must be added to the total cost for any node on the path which is not split. For our model we assume $t_{\text{overapprox}}<t_{\text{descend}}$ since the split needs to replicate the entire Zonotope and its connected state.
We can now take a more formal look at why CEGAR performs particularly bad.
CEGAR begins by computing an overapproximation based on the tree's root node and then tries to prove the property $\mathcal{E}$ at hand. If it fails, it branches on the root node and retries.
This strategy is performed iteratively until each path is successful.
Thus, CEGAR reaches the minimum number $P^*$ of paths to consider.
However, it comes with serious drawbacks: The check function is called significantly more often.
Additionally, for the $i$th refinement $p-i$ of the path's nodes need to be over-approximated.
Through the Gaussian sum we obtain a quadratic number of over-approximations.
This leads to the following lower bound for the algorithm's cost:
\[
\Omega\left(\sum_{p\in P^*} \left|p\right|*(t_{\text{check}}+t_{\text{descend}}) + \left|p\right|^2*t_{\text{overapprox}}\right)
\]
Note, that this is a lower-bound because we omit the cost $t_{\text{overapprox}}$ for the nodes which are over-approximated after we reach the necessary level of over-approximation in $P^*$.
Even when assuming the approximation to be free (i.e. $t_{\text{overapprox}}=0$) this approach becomes less effective than exact propagation once $\sum_{p\in P^*} \left|p\right| > \left|P\right|$.
While there are cases where this approach is effective, this is not always guaranteed to be the case -- especially for larger networks.

The optimal approach would use an oracle which tells the algorithm the number of refinement steps necessary for verifying $\mathcal{E}$ on the given path (i.e. $\min_{\mathcal{E}}$.
Assuming $t_{\text{overapprox}}=0$, the algorithm's cost would reduce to:
\[
\mathcal{O}\left(\left|P^*\right|*t_{\text{check}} + \sum_{p\in P^*} \left|p\right| * t_{\text{descend}}\right)
\]
It follows from the definition of $P^*$ that $\left|P^*\right| \leq \left|P\right|$ and that the average path length of $P^*$ is certain to be shorter or equal to the average length in $P$.
This implies that the oracle based algorithm would be certain to perform better than exact Zonotope GPE.
\todo{We could support this argument by experimentally running the oracle version (step 1: run CEGAR, step 2: run oracle version)}

It is thus important to find a good trade-off between the number of paths to consider and the number of operations necessary per path.
While the exact Zonotope approach yields a large number of paths at a comparatively low cost per path, the CEGAR approach yields the minimal number of paths at a very high cost per path.
We therefore explored a number of heuristics which are trying to estimate the minimum path length.
Again assuming $t_{\text{overapprox}}=0$ it is clear that a too low estimate produces additional checks while a too high estimate produces additional paths which need to be verified -- both either influencing the cost per path or the number of paths considered.
To this end we explored the following options:
\begin{enumerate}
    \item Maximum?
    \item Average*x?
    \item Running Average?
    \item Running Maximum?
    \item Running 95 percentile?
    \item Last Value
    \item Last Value - 1
\end{enumerate}

These strategies are much more difficult to analyze theoretically because they are particularly dependent on the distribution of the encountered paths and would thus only allow a probabilistic analysis for which we would then have to assume a probability distribution on the paths.

Maybe instead just give a rationale why we think certain strategies work better or worse?

\subsection{OLD}
We consider the algorithm in \Cref{algorithm:tree-exploration} which explores a binary tree.
At every node the algorithm has the possibility to either further descend into the tree in a depth first manner, or the algorithm can attempt to use an over-approximation.
This decision is made by the function \texttt{do\_approx}.
If the over-approximation is successful (executed and returned by \texttt{approx\_succ}, the algorithm must not further explore the current branch.
On the other hand, if the over-approximation fails, we must further \texttt{descend} into the children of the current node.
Both operations, descend and over-approximation check, come at a cost and it is thus necessary to find an optimal strategy which reduces the total cost of the tree exploration.
The tree nodes correspond to the neurons which we may either split on or over-approximate.
\todo{Only include this algorithm if it actually turns out to be interesting of course...}
\begin{algorithm}
    \caption{Tree Exploration Algorithm}
    \label{algorithm:tree-exploration}
    \begin{algorithmic}
    \REQUIRE Tree root $R$
    \ENSURE All branches explored or over-approximated
    \STATE $S \leftarrow \langle R \rangle$
    \WHILE{$\neg\texttt{S}.\texttt{empty}$}
        \STATE $n \leftarrow \texttt{S.pop}\left(\right)$
        \IF{$\texttt{do\_approx}\left(n\right)$\&\&$\texttt{approx\_succ}\left(n\right)$}
            \STATE \textbf{continue}
        \ENDIF
        \STATE $l,r \leftarrow \texttt{descend}\left(n\right)$
        \STATE $\texttt{S.pushAll}\left(\langle l,r \rangle\right)$
    \ENDWHILE
    \end{algorithmic}
\end{algorithm}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/acas-succ-depth.png}
    \caption{ACASXU\_run2a\_1\_1: Descend depth at point of successful equivalence proof for $\epsilon=0.05$ (Running percentile window: 479)}
    \label{fig:success-depth}
\end{figure}
In order to find the optimal positions for an over-approximation, we can execute the previously outlined naive refinement loop which iteratively refines more and more nodes from the start.
We can then track the number of \texttt{descend} operations which were necessary before \texttt{approx\_succ} was successful.
Consider the example of two ACAS Xu networks, a benchmark previously used for equivalence verification by \textcite{paulsen2020neurodiff}.
In \Cref{fig:success-depth} we show the number of necessary splits and some running percentiles for the Zonotopes considered during the equivalence verification of an ACAS Xu network, previously considered for equivalence verification by \textcite{paulsen2020neurodiff}.\todo{Since we talk about how \textcite{10.1007/978-3-030-76384-8_2} only used ACAS, we may want to use an MNIST -- at least additionally}.
The x axis represents the Zonotopes sequentially encountered over the runtime of the algorithm while the y axis describes the number of necessary refinement steps.
As can be seen from the data there is a high variance in the number of splits even locally. However, at the same time we see that the moving percentiles vary over time, thus indicating that certain \textit{phases} of the path enumeration require more splits than others.
This raises the question how the necessary number of refinement steps can be analyzed or, ideally, predicted based on previously encountered data.

Approaches considered so far:
\begin{itemize}
    \item Compute overall maximum. Problem: Does not fall once maximum was reached
    \item Take Last
    \item Take Last - 1
    \item Take Last - 2 (this one seemed worse)
    \item Take 95 percentile of last 300 or so(?)
    \item Taking running max of last 300 or so
\end{itemize}

==> old/sections/experiments.tex <==
Our qualitative experimental evaluation aims to answer the following questions:
\begin{itemize}
    \item[(E1)] Can the optimizations proposed above help in proving equivalence efficiently?
                Which speedup could maximally be achieved simply by finding better refinement heuristics?
    \item[(E2)] How large is the influence of the employed LP solver back-end? Does the Top-1 encoding by \textcite{Buning2020} significantly improve solving time?
    \item[(E3)] How does our approach compare to the approach by \textcite{Buning2020} for equivalence proofs as well as counter-example finding?
\end{itemize}
In order to answer these questions, we implemented our approach together with the optimizations outlined above building on the implementation by \textcite{bak2020improved}.
We then observed the behavior of our implementation and compared the results to the implementation by \textcite{Buning2020}.
\todo{Work on wording}
Note, that we decided not to compare our solution to the approach by \textcite{paulsen2020neurodiff}:
While our approach cannot compete with the results produced by \textcite{paulsen2020neurodiff}, a comparison would also be unfair due to the fact that our techniques apply to a more general category of networks (i.e. networks with potentially differing structures).

For the evaluation we chose to select a number of representative benchmark examples, some of which were previously presented in the literature some of which are new.
To this end, we built upon the MNIST network benchmarks used by \textcite{Buning2020} and modified versions of ACAS\_Xu networks presented by \textcite{julian2016policy} and previously used in the literature on neural network verification (e.g.~\cite{katz2017reluplex,bak2020improved}).
The secondary networks were either already given (as the case for the small and medium size MNIST networks) or retrained with the same or a different architecture using variants of Student-Teacher training~\cite{hinton2015distilling}.
Of all networks considered we knew they were equivalent or non-equivalent on certain parts of the input space.

\subsection{Comparison of Optimizations \& Heuristics}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/preliminary-comparison.png}
    \caption{Time taken for the 8 equivalent benchmarks considered:...}
    \label{fig:my_label}
\end{figure}
Benchmarks: A1, A2, D, E, F
\begin{itemize}
    \item Naive exact star
    \item Zono
    \item Zono+LP feasibility (i.e. exact)
    \item Zono Overapprox+LP approximation
    \begin{itemize}
        \item CEGAR
        \item Optimal
        \item Last-1
        \item Running Max
    \end{itemize}
\end{itemize}

\subsection{$\epsilon$ tightness}
\todo{Insert plot}
\textbf{NOTE}
Why did NNEquivalence return that bound while I found a counterexample?

\subsection{Counterexample finding}
\textbf{NOTE}
This one is difficult...
I mean I could easily find 10 examples where NNEquiv "instantly" returns a counter-example.
What seems much harder is to find cases where it works a very long time and eventually does find a counter-example.
However logic dictates these cases should exist...
Should we include this anyway?
Should I try to "manipulate" a network to show this behavior?

\subsection{Gurobi vs GLPK?}
I have done \textbf{some} parameter tuning (using gurobi's tune function), but there's certainly more that could be done here...
Use optimal approach from previous section and compare
Benchmarks: A1, A2, D, E, F

% \subsection{Input Dimensionality?}
% Benchmarks A1, A2, B, C

\subsection{Comparison to \textcite{Buning2020}}
Top 1:



Depending on input space size we're better or worse...

% @book{tange_ole_2018_1146014,
%       author       = {Tange, Ole},
%       title        = {GNU Parallel 2018},
%       publisher    = {Ole Tange},
%       month        = Mar,
%       year         = 2018,
%       ISBN         = {9781387509881},
%       doi          = {10.5281/zenodo.1146014},
%       url          = {https://doi.org/10.5281/zenodo.1146014}
% }


==> old/sections/extending_gpe.tex <==
In our work, we extend the previously presented GPE approach to be applicable to multiple neural networks.
Our approach is based on a point wise correspondence between the output data structures of GPE for two neural networks.
To make our approach clear we will introduce transfer functions as a way of reasoning about star sets or zonotopes.
\begin{definition}
Let $\mathcal{N}$ be a neural network.
$T_\mathcal{N}$ is a transfer function which, given an input data structure $\Theta$, produces a set of output data structures reachable through $\mathcal{N}$ with input $\Theta$, such that
\[
\left\{g_\mathcal{N}\left(x\right) \mid x \in \llbracket \Theta \rrbracket \right\} \subseteq \bigcup T_\mathcal{N}\left(\Theta\right)
\]
We call $T_\mathcal{N}$ \textit{exact} if the two sides are equal. Otherwise $T_\mathcal{N}$ is an overapproximation.
\end{definition}

Based on above transfer functions, we can show that there is a correspondence between the output sets of two neural networks in GPE:

\begin{theorem}[Network Output Correspondence]
    Let $\mathcal{R},\mathcal{T}$ be two networks with their corresponding transfer functions $T_\mathcal{R}$, $T_\mathcal{T}$ and let $\Theta^i=\langle c^i, G^i, P^i \rangle$ be some input data structure.
    
    For any $\Theta^o_1 = \langle c^o_1, G^o_1, P^o_1 \rangle \in T_\mathcal{R}\left(\Theta^i\right)$ we get that:\\
    For any $\Theta^o_2 = \langle c^o_2, G^o_2, P^o_2\rangle \in T_\mathcal{T}\left(\langle c^i, G^i, P^o_1 \rangle\right)$:
    \[
    \left\{ \left( g_\mathcal{R}\left(x\right), g_\mathcal{T}\left(x\right)\right) \mid x \in \llbracket \langle c^i, G^i, P^o_2 \rangle \rrbracket \right\}
    \subseteq
    \llbracket\langle c^o_1, G^o_1, P^o_2 \rangle\rrbracket \times \llbracket\Theta^o_2\rrbracket
    \]
    The two sides are equal iff $T_\mathcal{R}$ and $T_\mathcal{T}$ are exact.
\end{theorem}

This in turn gives rise to the modified GPE algorithm outlined in \Cref{algorithm:gpe-equiv:high-level}.
We begin by feeding our input data structure $\langle c^i, G^i, P^i\rangle$ into the first network.
For every output star set $\langle c^o_1, G^o_1, P^o_1 \rangle$, we feed the input data structure with restricted predicate according to the output of the first network, i.e. $\langle c^i, G^i, P^o_1 \rangle$ into the second network and obtain $\langle c^o_2, G^o_2, P^o_2 \rangle$.
In the end, we can compare the two output tuples $\langle c^o_1, G^o_1\rangle$ and $\langle c^o_2, G^o_2 \rangle$ constrained by the predicate $P^o_2$.

\begin{algorithm}
    \caption{High-level path enumeration algorithm for equivalence checking}
    \label{algorithm:gpe-equiv:high-level}
    \begin{algorithmic}
    \REQUIRE Input $\Theta = \langle c^i, G^i, P^i \rangle$, Neural Networks $\langle\mathcal{R},\mathcal{T}\rangle$
    \ENSURE Verification result (\texttt{equiv} or \texttt{nonequiv})
    \STATE $s \leftarrow \left\langle \texttt{network}:1, \texttt{layer}:0, \texttt{neuron}: \texttt{None}, \Theta: \Theta \right\rangle$
    \STATE $i \leftarrow \Theta$
    \STATE $\texttt{W} \leftarrow \texttt{List}()$ \COMMENT{List of set datastructures to process}
    \STATE $\texttt{W}.\texttt{put}\left(s\right)$
    \WHILE{$\neg\mathcal{W}$.\texttt{empty}()}
        \STATE $s \leftarrow \texttt{W}.\texttt{pop}()$
        \STATE $\texttt{step}_{s.\texttt{network}}\left(s, \texttt{W}\right)$
        \COMMENT{Next step in network ($\mathcal{R}$ or $\mathcal{T}$)}
        \IF{$s$ finished network 2}
            \STATE $\Theta^o_\mathcal{R} \leftarrow \langle s.\Theta^o_1.c, s.\Theta^o_1.G, s.\Theta^o_2.P \rangle$
            \STATE $\Theta^o_\mathcal{T} \leftarrow \langle s.\Theta^o_2.c, s.\Theta^o_2.G, s.\Theta^o_2.P \rangle$
            \IF{$\neg\texttt{is\_equiv}\left(\Theta^o_\mathcal{R},\Theta^o_\mathcal{T}\right)$}
                \RETURN \texttt{not equivalent}
            \ENDIF
        \ELSE
            \IF{$s$ finished a network 1}
                \STATE $s.\Theta^o_{s.\texttt{network}} \leftarrow s.\Theta$
                \STATE $s.\texttt{network}++$
                \STATE $s.\Theta \leftarrow \langle i.c, i.G, s.\Theta.P \rangle$
                \STATE $s.\texttt{layer}, s.\texttt{neuron} \leftarrow 0, \texttt{None}$
            \ENDIF
            \STATE $\texttt{W.push}\left(s\right)$
        \ENDIF
    \ENDWHILE
    \RETURN \texttt{equivalent}
    \end{algorithmic}
\end{algorithm}

Notice, that this scheme allows considering more than two networks, however, this work will be limited to the case of two networks.

\subsection{Equivalence on Set Data Structures}
While step functions can, in principle, be reused from previous works on GPE, it becomes necessary to define an equivalence check \texttt{is\_equiv} comparing two set data structures.
To this end we will, first, present how $\epsilon$-equivalence with Chebyshev norm $\left| \cdot \right|_\infty$ can be proven for Zonotopes.
Afterwards we will show how Star Sets can be used to prove a tighter variant of $\epsilon$-equivalence and top-1 equivalence.

\paragraph{$\epsilon$ Equivalence}
In order to prove $\epsilon$ equivalence with the Chebyshev norm, we need to bound the maximum deviation between the two network outputs by $\epsilon$.
That is, given the two output Zonotopes $\Psi^o_1 = \langle c^o_1, G^o_1, P^o_2 \rangle$ and $\Psi^o_2 = \langle c^o_2, G^o_2, P^o_2 \rangle$ we want to find the maximal deviation:
\begin{align*}
    &\max_{\alpha \in P^o_2} \left|\left(c^o_1+G^o_2 \alpha\right) - \left(c^o_2 + G^o_2 \alpha\right)\right|_\infty\\
    = &\max_{\alpha \in P^o_2} \max_{i} \left|\left(c^o_1-c^o_2\right)_i + \left(G^o_1-G^o_2\right)_i \alpha\right|.
\end{align*}
As can be seen by the reformulation above, we can find the maximal deviation over the output by solving optimization problems for each dimension of the \textit{differential Zonotope}
\[
\partial\Psi = \langle \left(c^o_1-c^o_2\right), \left(G^o_1-G^o_2\right), P^o_2 \rangle).
\]
Recalling, that Zonotopes can be optimized with a closed formula, this enables a relatively quick check for the adherence of the desired $\epsilon$ equivalence property.
However, since Zonotopes only approximate the output set, one may need to fall back to the use of Star Sets if equivalence cannot be established using Zonotopes.
In this case, we can reuse the same formula form above to obtain a \textit{differential star set} $\partial\Theta$ which is then optimized using LP solving.

\paragraph{Top 1 Equivalence}
For the case of Top 1 equivalence there are two possible approaches which both rely on propapagated star sets.
On the one hand, we can reuse the encoding by \textcite{Buning2020} using a MILP solver.\todo{Will we try this?}
If, on the other hand, we prefer to use a simplex solver, we can split up the output star sets further thus enabling us to establish Top 1 equivalence.
In this case we solve one optimization problem per output dimesion $j$.
To this end, for an $O$ dimensional output, we generate $O-1$ constraints which ensure that that dimension $j$ is the maximum in $\Theta^o_1$ and add those constraints to our second output $\Theta^o_2$.
We then compute the maximal difference between output dimension $j$ and the other dimensions in the modified version of $\Theta^o_2$.
In this case we must ensure that the maximal difference is always below $0$ to guarantee top 1 equivalence.
Top k equivalence follows trivially by allowing a certain number of dimensions above $0$.

\subsection{Challenges of the naive approach}
While the techniques outlined above, permit a straight forward extension of GPE to multiple networks and thus allow achieving equivalence verification, the approach comes with a number of pitfalls which one must avoid for the approach to succeed.
The most obvious of which is probably the, possibly, increased exponential growth in star sets.
As previously noted, the exact GPE approach based on star sets, splits the star sets on ReLU nodes and thus can yield a high rate of exponential growth.
\textcite{tran2019star} rightly noted that the observed growth usually drastically falls behind the worst case, however the increase in ReLU nodes certainly leads to an increase in necessary splits.
This is particularly the case for ReLU nodes which cut off very similar hyperplanes (such as the two ReLU nodes in a network at the same position with truncated weights).
This can not only double the work, but it may sometimes also lead to precision problems with typically used LP solvers which tend to show problematic behavior when encountering a problem which has two "nearly inversed" hyperplanes as bounds\footnote{In one case the solver would return drastically differing maximum values for the same optimization problem depending on the previous requests or would suddenly deem the problem infeasible.}.
To avoid such numerical problems we thus use 64bit floats by default and always ensure that feasibility is checked at least once by an exact (i.e. rational) LP solver before a branch is declared infeasible.
While these initial improvements help in making GPE for equivalence \textit{possible}, this approach is not yet \textit{scalable}.
Hence, we will devote the next section to various optimizations which we applied to improve the scalability of the approach.

==> old/sections/optimizing_gpe.tex <==
While the above stated approach does allow equivalence verification of very small input spaces, this approach is not yet scalable as the necessary LP optimizations and the number of considered splits for the exact case simply becomes too big to handle in a reasonable time frame.
Therefore we considered a number of optimizations, some of which have previously been used by \textcite{10.1007/978-3-030-76384-8_2}.

\subsection{Zonotope Propagation}
The first, most obvious, optimization is the use of overapproximating Zonotopes instead of exact star sets.
To this end, we reuse the propagation algorithm previously proposed by \textcite{bak2020improved} which splits the Zonotope on $\relu$ nodes overlapping $0$ and contracts the Zonotope bounds based on the hyper plane that is currently being split.
While this approach reduces the time spent on optimization, it comes at the cost of an increased number of splits. This is, because the Zonotope is not an exact approach. This is particularly worrysome if the Zonotope is propagated through two networks as it may reproduce very similar splits in both networks thus leading to more Zonotopes which need to be considered.
\todo{Maybe we could show some example here. I believe ACAS Xu 1010 had like 75\% splits which were actually infeasible}

\paragraph{Reintroducing LPs for feasibility checks}
However, we can avoid this issue without reintroducing the previous time spent on optimization by carrying a star set with the Zonotope which collects the so far encountered constraints.
This is also useful, because we need to solve LP problems during the top 1 equivalence check which can be done with greater precision if the split constraints are taken into account.
To mitigate this problem we propagate, both, the overapproximate Zonotope and the exact star set.
This is similar to the strategy used by \textcite{bak2020improved}.
However, instead of using the Zonotope as a prefilter, which decides on which ReLU nodes it is even necessary to execute LP optimization, we do not use the star set for optimization during the propagation.
Instead, we only regularly check the feasibility of the constraint set under consideration and abort the further propagation of the datastructure in case the constraints have become unsatisfiable.
In terms of algorithmics, this only executes the first phase of the Simplex algorithm and thus avoids the, sometimes costly, optimization once an initial basis has been found.

\subsection{Zonotope Overapproximation}
Even with these initial optimizations the algorithm is still left with a large number of Zonotopes which have to be evaluated.
We thus have two options to further optimize the algorithm: We can either further reduce the time spent per Zonotope or we can try to reduce the number of Zonotopes which have to be considered.
In order to achieve the second objective, we can over-approximate certain $\relu$ splits through a methodology first presented by \textcite{Singh2018} and later reused by \textcite{10.1007/978-3-030-76384-8_2}: The idea is to introduce an additional dimension to the Zonotope and use it to form a parallelogram around the area covered by the $\relu$ node.
While this decreases the amount of Zonotopes to consider, it also increases the over-approximation error.
In particular, the over-approximation can lead to more $\relu$ nodes supposedly needing to be split.
In \Cref{fig:gpe-splitting} we compare the share of nodes per layer that are ever considered for a split or over-approximation for splitting Zonotope propagation in comparison with overapproximating Zonotope propagation for an ACAS Xu network:
As can clearly be seen in the plot, the overapproximation approach produces a lot more alleged splits than the exact approach.
These \textit{ghost splits} cannot be easily distinguished from actual, necessary splits.
Note that this comparison aggregates the number of splits over all splitted Zonotopes for the exact case -- for a single propagated Zonotope the number of splits is usually even lower.
This can in turn result in even more over-approximation error which \textcite{10.1007/978-3-030-76384-8_2} referred to as \textit{error snowball}.
Since the over-approximation of all $\relu$ nodes can result in a situation where the desired properties are no longer provable due to approximation error, it becomes necessary to find a suitable refinement heuristic which decides what nodes are refined if an equivalence property cannot be established.
We will discuss the search for a suitable refinement strategy in the next section, however there is one more efficiency improvement related to the dimensionality of the LP problems solved.

%\todo{Should we show this? reference in text? maybe also with mnist?}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/split-neurons-acas.png}
    \caption{Share of $\relu$ nodes per network layer which are ever split during GPE. (Overapprox Net1 is hidden behind Overapprox Net2)}
    \label{fig:gpe-splitting}
\end{figure}

\subsection{LP approximation}
With the introduction of over-approximation we encounter an additional problem: As splitting hyperplanes are now no longer dependent on the input variables \textit{only}, but also depend on the dimensions introduced through the over-approximation, it raises the question how to handle this situation in the propagated star set: Should the we equally introduce the star sets dimensionality and thus the dimensionality of the LP problem?
This strategy poses the problem that can increase the computational load on the LP solver.
Instead, we opted to overapproximate the LP problem.
Classically, for an $m$ dimensional Zonotope with initial input dimensionality $I$ we observe a hyperplane cut of the following form:
\begin{align}
\sum_{i=1}^I g_i \alpha_i + \sum_{i=I+1}^m g_i \alpha_i \leq c
\label{eq:exact-lp}
\end{align}
We can now over-approximate this pro inequality by computing $\mu = \min_{\alpha} \sum_{i=I+1}^m g_i$
and constraining the LP problem with the following inequality:
\begin{align}
    \sum_{i=1}^I g_i \alpha_i \leq c - \mu
    \label{eq:approx-lp}
\end{align}
Since any solution for \Cref{eq:exact-lp} implies a solution for \Cref{eq:approx-lp} the second inequality is an over-approximation and can be used to reduce the number of dimensions the LP solver has to handle despite the use of over-approximation on the GPE side.




==> old/sections/related_work.tex <==
In this section, we will briefly review works relevant to our research.
Firstly, we will give a short introduction to various equivalence properties before presenting current State-of-the-Art approaches in equivalence verification.
Subsequently, we will give an introduction of Geometric Path Enumeration for single networks that will be useful in the following sections.
\subsection{Verifiying Neural Network Equivalence}
There has recently been a line of work which proposed various compression techniques for neural networks (a full review of such the techniques was recently presented by \textcite{cheng2020survey}).
While such techniques have been shown to be useful in practice, most lack a formal proof of their correctness and rely on empirical evidence.
The usage of such techniques thus raises the question how to prove that two neural networks $\mathcal{R}$ and $\mathcal{T}$ or their corresponding mathematical functions $g_{\mathcal{R}}:\mathbb{R}^I\to \mathbb{R}^O, g_{\mathcal{T}}:\mathbb{R}^I\to \mathbb{R}^O$ are equivalent, i.e. that they produce the same results.
%we aim to answer the question whether the two networks are equivalent.
%It thus becomes necessary to precisely define what it means for two neural networks to be equivalent in order to check such properties.
To this end, \textcite{Buning2020} examined three possible definitions of equivalence in a predefined subset $X\subseteq \mathbb{R}^I$, two of which we will review here:\todo{Add top k?}
\begin{definition}[$\epsilon$-Equivalence\cite{Buning2020}]
\label{def:epsilon-equiv}
Two networks $\mathcal{R}$ and $\mathcal{T}$ are $\epsilon$-equivalent with respect to a norm $\lVert \cdot \rVert$, if $\left\lVert g_{\mathcal{R}}\left(x\right)-g_{\mathcal{T}}\left(x\right)\right\rVert \leq \epsilon$ for all $x \in X$
\end{definition}
%\todo{mkb: this property is checked by ReluDiff and called differential verification of NNs by them}
\begin{definition}[One-Hot Equivalence\cite{Buning2020}]
\label{def:one-hot-equiv}
Two networks $\mathcal{R}$ and $\mathcal{T}$ are one-hot equivalent, if $\argmax_i \left(g_{\mathcal{R}}\left(x\right)\right)_i = \argmax_i \left(g_{\mathcal{R}}\left(x\right)\right)_i$ for all $x \in X$
\end{definition}
%\Cref{def:one-hot-equiv} can be further relaxed by considering more than one label:
%\begin{definition}[Top-$k$ Equivalence\cite{Buning2020}]
%\label{def:top-k-equiv}
%Two networks $\mathcal{R}$ and $\mathcal{T}$ are top-$k$ equivalent, if given $g_{\mathcal{R}}\left(x\right)=r$ and $g_{\mathcal{T}}\left(x\right)=t$:
%\[
%\argmax_i r_i = j \implies \pos(t_j, t) \leq k
%\]
%where $\pos(v_j, v)$ returns $i$, if $v_j$ is the $i$-th largest value of $v$
%\end{definition}
While Definition \ref{def:epsilon-equiv} is particularly suitable for regression tasks as it can show a very strong form of equivalence, the latter definition represents a more relaxed interpretation of equivalence which can be especially useful for classification tasks.
\textcite{paulsen2020reludiff} refer to the property in Definition \ref{def:epsilon-equiv} as \textit{differential equivalence}.

\textcite{paulsen2020neurodiff} and \textcite{Buning2020} proposed two fundamentally different approaches to neural network equivalence verification with differing application areas.
While \textcite{paulsen2020neurodiff} propose a technique which uses (symbolic) interval propagation on structurally similar neural networks (i.e. networks with the same architecture but differing weights) to prove $\epsilon$ equivalence, \textcite{Buning2020} propose a technique based on Mixed Integer Linear Program solving which encodes (potentially) structurally differing neural networks and the desired equivalence property into an optimization problem.
While the approach by \textcite{paulsen2020neurodiff} was shown to be efficient for cases where a networks weights had been truncated, \textcite{Buning2020} showed that their approach can works well for a number of small networks and all previously mentioned equivalence properties (e.g. two 64 pixel MNIST networks with a total of 84 $\relu$ nodes).
In particular, \textcite{Buning2020} were able to provide a maximal radius around a datapoint for which the property still held.

\subsection{Geometric Path Enumeration}
Geometric Path Enumeration is a methodology originally proposed by \textcite{tran2019star} for verifying safety properties in neural networks.
Given a neural network $\mathcal{N}$, a set of input instances $\mathcal{I}\subseteq\mathbb{R}^I$ and a safety specification $\mathcal{S}\subseteq\mathbb{R}^O$, safety verification concerns with the question whether there exist any instances $i\in\mathcal{I}$ such that $g_{\mathcal{N}}\left(i\right) \notin \mathcal{S}$.
In their work, a safety specification $\mathcal{S}$ is defined as a set of linear constraints on the neural network outputs $\left\{y^{(L)} | C y^{(L)} \leq d\right\}$

\begin{algorithm}
    \caption{High-level path enumeration algorithm for neural networks as described in \cite{bak2020improved}}
    \begin{algorithmic}
    \label{algorithm:gpe-basics:high-level}
    \REQUIRE Input Set $\mathcal{I}$, Unsafe Set $\mathcal{U}$
    \ENSURE Verification result (\texttt{safe} or \texttt{unsafe})
    \STATE $s \leftarrow \left\langle \texttt{layer}:0, \texttt{neuron}: \texttt{None}, \Theta: \texttt{convert}\left(\mathcal{I}\right) \right\rangle$
    \STATE $\texttt{W} \leftarrow \texttt{List}()$ \COMMENT{List of set datastructures to process}
    \STATE $\texttt{W}.\texttt{put}\left(s\right)$
    
    \WHILE{$\neg\mathcal{W}$.\texttt{empty}()}
        \STATE $s \leftarrow \texttt{W}.\texttt{pop}()$
        \STATE $\texttt{step}\left(s, \texttt{W}\right)$
        \COMMENT{This call may modify \texttt{W} and $s$}
        \IF{$\neg \texttt{finished}\left(s\right)$}
            \STATE $\texttt{W.push}\left(s\right)$
        \ELSIF{$\neg \texttt{verify}\left(s, \mathcal{U}\right)$}
            \RETURN \texttt{unsafe}
        \ENDIF
    \ENDWHILE
    \RETURN \texttt{safe}
    \end{algorithmic}
\end{algorithm}

Instead of pushing single instances through the network and checking whether they satisfy the required safety property, geometric path enumeration feeds an entire set into the neural network and then evaluates whether any parts of the output sets lie outside the safety specification.
The general setup of this idea can be observed in Algorithm \ref{algorithm:gpe-basics:high-level}: The algorithm's input consists of an input set to evaluate and an unsafe set of states that should not be reached from the input set under consideration.
We then convert the input set into an internal data structure storing both a representation of the set and how far the set has been pushed through the network so far.
We add this data structure to a list \texttt{W} of sets to consider.
We then continuously push the data structures inside \texttt{W} through the neural network at hand using the \texttt{step} function until there are either no further sets to consider or an unsafe state has been observed in the network's final layer.

As data structure to be propagated throughout the network, the authors propose to use generalized star sets:
\begin{definition}[Generalized Star Set\cite{tran2019star}]
A generalized star set $\Theta$ is a tuple $\left\langle c, G, P\right\rangle$ where $c\in\mathbb{R}^n$ is the center, $G=\left\{g_1,\cdots,g_m\right\}$ is a set of $m$ vectors in $\mathbb{R}^n$ called basis vectors, and $P:\mathbb{R}^m \to \left\{\top,\bot\right\}$ is a predicate which is (in the works under consideration) restricted to be a conjunction of linear constraints.
%\todo{Sometimes also refered to as half space polytope if we prefer that name?}
The set represented by $\Theta$ is then defined as:
\[
\left\llbracket \Theta \right\rrbracket = \left\{ x \middle\vert x = c + \sum_{i=0}^{m-1} (\alpha_i v_i)\text{ such that } P\left(\alpha_1,\cdots,\alpha_m\right) \right\}
\]
\todo{indices in sum and predicate don't match}
We will sometimes also refer to $G$ as generator and as matrix $G=\left(g_1g_2\cdots g_m\right)$.
%For simplicity we denote $c + G\alpha$ as $\Theta\left(\alpha\right)$.
%For simplicity we will sometimes refer to $c + G\alpha$ as $\Theta\left(\alpha\right)$.
\label{def:gpe:star-set}
\end{definition}
Alternatively, it is possible to use Zonotopes which further restrict the type of predicate allowed:
\begin{definition}[Zonotopes\cite{bak2020improved}]
A Zonotope $\Psi$ is a generalized star set $\langle c, G, P \rangle$ with the further restriction that $P$ may only be an interval constraint (i.e. $P$ only enforces a lower and upper bound for each dimension).
\end{definition}

\Cref{algorithm:gpe-basics:high-level} can be completed by providing suitable \texttt{step}, \texttt{finished} and \texttt{verify} functions for the desired data structure as previously done by \textcite{tran2019star}.
Note that minimization/maximization for Generalized Star Sets is much more expensive than optimization for Zonotopes, which can be computed analytically.
While affine transformations can trivially be applied to both data structures, it is less clear how $\relu$ nodes should be handled by the datastructure.
To this end, one can either split the Zonotope into two cases or one can use various over-approximation techniques\cite{Singh2018,10.1007/978-3-030-76384-8_2}.
We call the approach which splits generalized star sets \textit{exact GPE} and other approaches \textit{approximate GPE} since Zonotopes are usually unable to provide an exact output.
